QDFormer: Towards Robust Audiovisual Segmentation in Complex Environments with Quantization-based Semantic Decomposition

Audiovisual segmentation (AVS) is a challenging task that aims to segment visual objects in videos according to their associated acoustic cues. With multiple sound sources and background disturbances involved, establishing robust correspondences between audio and visual contents poses unique challenges due to (1) complex entanglement across sound sources and (2) frequent changes in the occurrence of distinct sound events. Assuming sound events occur independently, the multi-source semantic space can be represented as the Cartesian product of single-source sub-spaces. We are motivated to decompose the multi-source audio semantics into single-source semantics for more effective interactions with visual content. We propose a semantic decomposition method based on product quantization, where the multi-source semantics can be decomposed and represented by several disentangled and noise-suppressed single-source semantics. Furthermore, we introduce a global-to-local quantization mechanism, which distills knowledge from stable global (clip-level) features into local (frame-level) ones, to handle frequent changes in audio semantics. Extensive experiments demonstrate that our semantically decomposed audio representation significantly improves AVS performance, e.g., +21.2% mIoU on the challenging AVS-Semantic benchmark with ResNet50 backbone. https://github.com/lxa9867/QSD.

==> src/_1-intro.tex <==
\section{Introduction}
Recent advances in prompt-guided video object segmentation \cite{kirillov2023segment,cheng2023segment} have showcased impressive capabilities in segmenting a single visual object based on visual regions (video object segmentation \cite{wang2023look,hong2023lvos}), text descriptions (referring video object segmentation \cite{wu2022language,wu2023onlinerefer}), and even auditory cues (audiovisual segmentation \cite{zhou2023audio,zhou2022avs}). However, the complexity escalates when multiple target objects coexist in a frame. Unlike visual regions or textual descriptions, which can be readily disentangled to characterize different objects, audio undergoes inevitable mixing, presenting a formidable challenge in segmenting objects with multi-source audio.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/teaser2.pdf}
\vspace{-0.5cm}
\caption{Our method addresses the multi-source AVS by decomposing audio features into several semantic tokens based on their corresponding video contents. The semantic decomposition utilizes product quantization (PQ) as an information bottleneck to achieve a compact while informative representation.
}
% , which employs a shared codebook to constrain the consistency and cardinality of each decomposed semantic subspace.}
\vspace{-0.4cm}
\label{fig:teaser2}
\end{figure}

Previous attempts \cite{zhou2022avs,li2023catr,gao2023avsegformer} mostly address the multi-source audiovisual segmentation problem by drawing inspiration from text-queried segmentation methods \cite{referformer,botach2022end}, which directly interact the multi-source audio with visual contents. However, this can result in suboptimal performance for two primary reasons. (1) \textit{Entangled multi-source audio semantics}: Unlike the visual domain, where each pixel is associated with a single semantic label, an audio timestamp can correspond to multiple sources with a combination of semantic labels, resulting in alignment ambiguity between audio and visual elements. Effective audiovisual interaction necessitates the decomposition of entangled audio features. (2) \textit{Background disturbances}: In contrast to textual expression, which contains unambiguous information to identify objects, acoustic cues are inherently vulnerable to disturbances from background noises. Consequently, a compact and task-relevant representation that discards unnecessary entangled details is crucial.



\begin{figure}[t]
\centering    
\includegraphics[width=\linewidth]{figs/teaser_cvpr24.pdf}
\vspace{-0.7cm}
    \caption{(a) \textbf{Audiovisual semantic interaction.} In the single-source moments, only singing or guitar sound is active; In the multi-source moment, both singing and guitar are simultaneously active. In the whole clip, visual semantic content remains consistent. (b) \textbf{Semantic decomposition.} Multi-source audio semantic space can be assumed as a Cartesian product of single-source semantics, which can be decomposed via product quantization by constraining the codebook size smaller than the semantic space size. The {\color{red}{red}} points represent the quantized semantics.
    }
    %\vspace{-0.2cm}
\label{fig:teaser_decompose}
\end{figure}

As shown in \cref{fig:teaser2}, we propose to leverage audio quantization to achieve a more robust representation and disentangle the multi-source audio semantics to enable more effective audiovisual interaction. Specifically, we introduce the information bottleneck for audio representation as
it can (1) find a compact and task-relevant representation that discards unnecessary entangled details \cite{tishby2000information}, (2) guide disentanglement, aiding in separating the underlying factors of audio in a more effective and interpretable manner~\cite{alemi2016deep,achille2018emergence}, (3) facilitate more efficient matching and comparison of features by converting high-dimensional features into discrete symbols.
Specifically, we introduce a Product Quantization (PQ) based method to decompose multi-source semantics with its capability to represent a complex space through the product of several subspaces \cite{jegou2010product}. 
As shown in \cref{fig:teaser}, we define that the set of all potential semantic labels of pixels corresponds to the \textit{visual semantic space}, and the label set of acoustic timestamps corresponds to the \textit{acoustic semantic space}. During single-source moments (left of \cref{fig:teaser} (a)), it is evident that the visual semantic space corresponds to the semantic labels $\mathcal{Y} = $ \{Guitar (G), Singing (S)\}, and the acoustic semantic space are of an identical label set $\mathcal{Y}$. Moving on to the two-source moment (right of \cref{fig:teaser} (a)), the visual semantic space remains consistent with previous frames, but the \textit{possible} two-source audio semantic space expands to a misaligned $\mathcal{Y} \times \mathcal{Y} = $\{GG, GS, SG, SS\}. To solve this, we simplify the problem by assuming independent sound events, which allows us to represent the multi-source semantic space as a Cartesian product of identical single-source semantic spaces. With product quantization as an information bottleneck (which can be achieved by utilizing a shared codebook to quantize as illustrated in \cref{fig:teaser2}), we can decompose the multi-source audio semantics into single-source semantics as shown in \cref{fig:teaser} (b). 

Furthermore, it is necessary to analyze audio semantics for every frame, given that sounding sources can change frequently. This presents a robustness challenge, as extracted semantics from short-term audio can be unstable compared to the extraction from long-term (clip-level) audio. To improve the frame-level audio representation, we propose a global-to-local mechanism, which distills knowledge from robust global (clip-level) audio representations into local (frame-level) ones.
Specifically, we build an effective codebook for semantic quantization with clip-level visual-enriched audio features and then apply this codebook to perform local quantization on each frame without updating it. Thereby, the local semantic tokens are calibrated to the more robust and representative clip-level feature in the codebook.

In summary, our contribution is three-fold: 
\begin{itemize}
    \item An effective approach of multi-source audio semantic decomposition via product quantization, addressing the challenge of interacting visual and audio features in multiple object scenarios.     
    \item A global-to-local distilling mechanism for frame-level audio semantic enhancement, addressing the ineffectiveness of frame-level audio feature extraction.
    \item Extensive experiments are conducted to verify the effectiveness and robustness of the proposed method, which significantly outperforms previous state-of-the-art methods on three AVS benchmarks (+21.2\% mIoU for AVS-Semantic).
\end{itemize}

% We depict the PQ-based semantic decomposition of a two-source example in \cref{fig:teaser} where 
% PQ can be easily achieved by learning separate transforms of multi-source semantics and then quantizing them utilizing a shared codebook as illustrated in \cref{fig:teaser2}. 

% Let us start explaining the high-level idea with a basic scenario involving a single sound source (left of \cref{fig:teaser} (a)). 
% In this context, each pixel and each timestamp are associated with only one semantic label.
% We define that the set of all potential semantic labels of pixels corresponds to the \textit{visual semantic space}, and the label set of acoustic timestamps corresponds to the \textit{acoustic semantic space}.
% During single-source moments, it is evident that the visual semantic space corresponds to the semantic labels $\mathcal{Y} = $ \{Guitar (G), Singing (S)\}, and the acoustic semantic space are of an identical label set $\mathcal{Y}$.
% Moving on to the two-source moment (right of \cref{fig:teaser} (a)), the visual semantic space remains consistent with previous frames, but the \textit{possible} two-source audio semantic space expands. We simplify the problem by assuming independent sound events, which allows us to represent the multi-source semantic space as a Cartesian product of identical single-source semantic spaces. Thus the audio semantic space corresponds to $\mathcal{Y} \times \mathcal{Y} = $  \{GG, GS, SG, SS\}, with a quadratic expansion.
% This not only escalates the challenge of modeling larger semantic spaces but also complicates the task of aligning visual and acoustic semantic spaces. The complexity further amplifies as the number of audio sources increases.

% The recent emergence of audiovisual segmentation (AVS) \citep{zhou2022avs} presents a promising approach to explore audiovisual correlations at the pixel level.
% AVS targets the segmentation of sounding objects within video frames with their associated audio as prompt. Building on it, audiovisual semantic segmentation (AVSS) \citep{zhou2023audio} extends the task by additionally determining the categories of the segmented masks, as shown in \cref{fig:teaser} (a). 



% Notably, the annotation only includes separate masks, not separated audio for multiple sounding sources.
% Unlike the visual domain where each pixel is associated with a single semantic label, an audio timestamp can correspond to multiple sources with different semantic labels, resulting in alignment ambiguity between audio and visual elements.
% This motivates us to explore appropriate representations for multi-source audio to achieve more effective audiovisual interactions.





% \cb{
% Let us start by examining the most basic scenario (left of \cref{fig:teaser} (a)) involving a single sound source. In this context, each pixel and each timestamp are associated with only one semantic label.
% We define that the set of all potential semantic labels of pixels corresponds to the \textit{visual semantic space}, and the label set of acoustic timestamps corresponds to the \textit{acoustic semantic space}.
% During single-source moments, it is evident that the visual semantic space corresponds to the semantic labels $\mathcal{Y} = $ \{Guitar (G), Singing (S)\}, and the acoustic semantic space are of an identical label set $\mathcal{Y}$.
% Moving on to the two-source moment (right of \cref{fig:teaser} (a)), the visual semantic space remains consistent with previous frames, but the \textit{possible} two-source audio semantic space expands. We simplify the problem by assuming independent sound events, which allows us to represent the multi-source semantic space as a Cartesian product of identical single-source semantic spaces. Thus the audio semantic space corresponds to $\mathcal{Y} \times \mathcal{Y} = $  \{GG, GS, SG, SS\}, with a quadratic expansion.
% This not only escalates the challenge of modeling larger semantic spaces but also complicates the task of aligning visual and acoustic semantic spaces. The complexity further amplifies as the number of audio sources increases.
% } \ca{semantic space, label set or feature? conflict with 3.1}


% Previous AVS methods \citep{zhou2023audio,zhou2022avs,yuanhong2023closer} directly correlate entangled audio with visual content, which leads to increased complexity and difficulty introduced by multi-source audio.
% We propose to disentangle the multi-source audio semantics into several single-source ones to enable more effective audiovisual interaction. Although separating audio in advance with a pretrained model is an alternative, it cannot be fine-tuned on AVS(S) datasets due to the absence of separated audio annotations. 
% Hence, our solution is to achieve audio decomposition effectively by interacting with visual features while being supervised by separate masks.
% We leverage information bottleneck for audio semantic decomposition as
% it can 1) find a compact and task-relevant representation that discards unnecessary entangled details \cite{tishby2000information}, 2) guide disentanglement, aiding in separating the underlying factors of audio in a more effective and interpretable manner~\cite{alemi2016deep,achille2018emergence}, 3) facilitate more efficient matching and comparison of features by converting high-dimensional features into discrete symbols.
% Specifically, we introduce a Product Quantization (PQ) based method to decompose multi-source semantics as PQ can represent a complex space through the product of several subspaces \cite{}. 
% We depict the PQ-based semantic decomposition of a two-source example in \cref{fig:teaser} (b). 
% Moreover, PQ can be easily achieved by learning separate transforms of multi-source semantics and then quantizing them utilizing a shared codebook as illustrated in \cref{fig:teaser2}. 





==> src/tab_ab_pre.tex <==


\begin{table*}
\centering
%\captionsetup{justification=raggedleft,singlelinecheck=false}
\scalebox{1}{
\begin{tabular}{lp{1.4cm}
<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}|p{3cm}<{\centering}} 
\hline
\multirow{2}*{Module} & \multicolumn{3}{c}{AVS-Object-Multi} & AVS-Sementic\\
\cline{2-5}
~ & $\mathcal{J} \& \mathcal{F}\uparrow$ & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$ & mIoU$\uparrow$\\
\hline
Baseline (no decomposition) & 52.9 & 50.1 & 55.7 & 33.5 \\
\hline
+GSD & 56.7 & 54.5 & 58.8 & 38.4\\
+GSD+AVSR & 58.6 & 56.5 & 60.6 & 40.9\\
+GSD+AVSR+LSD & 60.1 & 58.2 & 61.9 & 44.5\\
\rowcolor{verylightgray}+GSD+AVSR+LSD+SC & 61.6 & 59.6 & 63.5 & 46.6 \\
no quantization (+GSD+AVSR+LSD-CB)  & 58.6 & 57.1 & 60.1 & xx \\
\hline
\end{tabular}
}
\caption{Component analysis. GSD: global semantic decomposition; AVSR: audiovisual semantic recombination; LSD: local semantic decomposition; SC: sharing codebook. \ca{delete}}
\label{tab:module effectiveness}
\end{table*}



\begin{table*}[t]
\begin{minipage}[t]{\textwidth}
\begin{minipage}[t]{0.28\textwidth}
\makeatletter\def\@captype{table}
\centering
\scalebox{0.85}{
\begin{tabular}{cp{1.4cm}
<{\centering}p{1.4cm}<{\centering}} 
\hline
{Codebook } &
Object-M & Sementic\\
\cline{2-3}
Size & $\mathcal{J} \& \mathcal{F}\uparrow$ & mIoU$\uparrow$\\
\hline
1 & 52.7 & 24.8\\
32 & 61.4 & 31.5\\
64 & 60.0 & 43.2 \\
\rowcolor{verylightgray}128 & 61.6 & 46.6\\
256 & 60.6 & 46.1 \\
\hline
\end{tabular}
}
\caption{Ablation on codebook size.}
\label{tab:codebook size}
\end{minipage}
\hspace{0.04\textwidth}
\begin{minipage}[t]{0.32\textwidth}
\makeatletter\def\@captype{table}
\centering
\scalebox{0.85}{
\begin{tabular}{cp{2.0cm}
<{\centering}p{2.0cm}<{\centering}} 
\hline
{Token } &
Object-M & Sementic\\
\cline{2-3}
Number & $\mathcal{J} \& \mathcal{F}\uparrow$ & mIoU$\uparrow$\\
\hline
1 & 59.7 & 40.2 \\
3 & 61.0 & 43.5 \\
\rowcolor{verylightgray}5 & 61.6 & 46.6 \\
7 & 61.6 & 45.9 \\
9 & 61.2 & 46.3 \\
\hline
\end{tabular}
}
\caption{Ablation on decomposed token number.}
\label{tab:token number}
\end{minipage}
\hspace{0.04\textwidth}
\begin{minipage}[t]{0.26\textwidth}
\makeatletter\def\@captype{table}
\centering
\scalebox{0.85}{
\begin{tabular}{cp{1.4cm}
<{\centering}p{1.4cm}<{\centering}} 
\hline
{Decomp.} &
Object-M & Sementic\\
\cline{2-3}
Domain & $\mathcal{J} \& \mathcal{F}\uparrow$ & mIoU$\uparrow$\\
\hline
Time & 56.2 & 38.9\\
\rowcolor{verylightgray}Semantic & 61.6 & 46.6\\
\hline
\end{tabular}
}
\caption{Ablation on sound decomposition domain.}
\label{tab:decompose}
\end{minipage}
\end{minipage}
\end{table*}
